Giving Back: Contributions Congruent to Library Dependency Changes in a Software Ecosystem

Popular adoption of third-party libraries for contemporary software development has led to the creation of large inter-dependency networks, where sustainability issues of a single library can have widespread network effects. Maintainers of these libraries are often overworked, relying on the contributions of volunteers to sustain these libraries. In this work, we measure contributions that are aligned with dependency changes, to understand where they come from (i.e., non-maintainer, client maintainer, library maintainer, and library and client maintainer), analyze whether they contribute to library dormancy (i.e., a lack of activity), and investigate the similarities between these contributions and developers' typical contributions. Hence, we leverage socio-technical techniques to measure the dependency-contribution congruence (DC congruence), i.e., the degree to which contributions align with dependencies. We conduct a large-scale empirical study to measure the DC congruence for the NPM ecosystem using 1.7 million issues, 970 thousand pull requests (PR), and over 5.3 million commits belonging to 107,242 NPM packages. At the ecosystem level, we pinpoint in time peaks of congruence with dependency changes (i.e., 16% DC congruence score). Surprisingly, these contributions came from the ecosystem itself (i.e., non-maintainers of either client and library). At the project level, we find that DC congruence shares a statistically significant relationship with the likelihood of a package becoming dormant. Finally, by comparing source code of contributions, we find that congruent contributions are statistically different to typical contributions. Our work has implications to encourage and sustain contributions, especially to support library maintainers that require dependency changes.

==> sections/OLDmethodology.tex <==


% \section{Aligning Contributions And Dependencies}\label{sec:methodology}

% Based on the preliminary analysis, we now define ecosystem congruence to understand the extent to which contributions are performed in congruence with their dependencies.


\begin{table*}[t]
\caption{Graph Edge Attributes.}
\label{tab:data-statistic}
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{}                    & \textbf{Attribute} & \textbf{Type}     & \textbf{Description}                                                                                                                                       \\ \midrule
\multicolumn{1}{l|}{$E_{c}$} & E.role             & is-maintainer     & A developer who has the ability to merge any submitted contributions.                                                                                      \\
\multicolumn{1}{l|}{}        & E.role             & is-non-maintainer & \begin{tabular}[c]{@{}l@{}}A developer who can only submit contributions to a package, \\ but does not have the ability to merge the package.\end{tabular} \\ \midrule
\multicolumn{1}{l|}{$E_{d}$} & E.state            & is-added          & A dependency has just been added.                                                                                                                          \\
\multicolumn{1}{l|}{}        & E.state            & is-removed        & A dependency has been removed from a package.                                                                                                              \\
\multicolumn{1}{l|}{}        & E.state            & is-upgraded       & A dependency version has been changed to a more recent version.                                                                                            \\
                             & E.state            & is-downgraded     & A dependency version has been changed to an older version of a library.                                                                                    \\ \bottomrule
\end{tabular}
\end{table*}
% \subsection{Modeling Contribution and Dependency}
\subsection{Graph Representation}
Figure \ref{fig:graph} is a visual example of our definition of aligning contributions and dependencies in the ecosystem.
Let $G = (N, E)$ for a directed graph $G$.
N has two types of nodes, where $N_{dev}$ refers to a developer, while $N_{pkg}$ refers to a software package.
$N_{pkg}$ has attributes <name, time> where name is the unique name of the package and time is when the package was first created.
$N_{dev}$ has an attribute <userid> where userid is the unique identification of the developer.
Since we capture the contributions and dependencies, there are two types of edges in our graph. 

\begin{definition}[Contribute $N_{dev} \Rightarrow N_{pkg.i}$]
The second \christoph{first} is $E_{c}$, which is an edge between a $N_{dev}$ and a $N_{pkg.i}$, where a developer $N_{dev}$ contributes to a package $N_{pkg.i}$. 
Note that a package cannot contribute to a developer (i.e., $N_{pkg.i} \Rightarrow N_{dev}$ does not exist).
% \christoph{Make it explicit here that this edge is also directed, and can only exist in the dev to pkg direction, not the other way around}
\end{definition}

\begin{definition}[Depend  $N_{pkg.i} \rightarrow N_{pkg.j}$]
The first \christoph{second} is $E_{d}$, which is an edge between two $N_{pkg}$, representing a dependency relationship between the two packages.
Since this is a directed graph, there is a direction of the edge where $N_{pkg.i} \rightarrow N_{pkg.j}$ is where package i ($N_{pkg.i}$) is a client that depends on the library package j ($N_{pkg.j}$).
\end{definition}



\subsection{Contributor Role and Dependency State Attributes}
The graph also has temporal and state attribute information relating to the contributions and dependency alignment. \christoph{Maybe make it explicit that it's the edges that have these attributes?}
% \begin{figure}[t]
%     \centering
%     \scalebox{0.9}{
%     \begin{tikzpicture}[
%         roundnode/.style={circle, fill=black, minimum size=5mm},
%         squarenode/.style={fill=cyan, text=red, minimum size=5mm},
%     ]
%     \begin{scope}
        
%         \node[roundnode, label=right:$Pkg\_i$ as client] (s2_proji) at (4, 3) {};
%         \node[roundnode, label=below:$Pkg\_j$ as library] (s2_projj) at (4,0) {};

%         \node[squarenode, label=below:$Dev\_x$] (s3_devx) at (1.5, 1.5) {};
        
        
%     \end{scope}

%     \begin{scope} [every edge/.style={draw=red, very thick},
%     every node/.style={fill=white}]
%         \path [->] (s2_proji) edge[bend left=70] node {\textbf{depend}} (s2_projj);
        
%     \end{scope}
%     \begin{scope} [every edge/.style={draw=gray, ultra thick},
%     every node/.style={fill=white}]
%         \path [->] (1.9, 1.5) edge[bend left=35] node {contribute as \textbf{maintainer}} (s2_proji);
%         \path [->] (1.9, 1.5) edge[bend right=35] node {contribute as \textbf{maintainer}} (s2_projj);
%     \end{scope}
%     \end{tikzpicture}
%     }
%     \caption{Co-maintainer contributions}
%     \label{fig:contribue-m}
% \end{figure}

% \paragraph{\textbf{Contribute-d}} - We now calculate the congruence based on a developer that has a dependency. 

% \paragraph{\textbf{Contribute-m}} - We now calculate the congruence based on a developer that has a dependency. 
% \begin{enumerate}[{\bf DC3:}]
%   \item DC$_{t1-t2}$ = $\frac{Match(Dep_{t1-t2}, ConMaintain_{t1-t2})}{|Dep_{t1-t2}|}$
% \end{enumerate}

% Where $Dep_{t1-t2}$ is the Ecosystem dependency matrix and $ConMaintain_{t1-t2}$ is the Maintainer matrix.

% \begin{enumerate}[{\bf DC4:}]
%     \item DC$_{t1-t2}$ = $\frac{Match(DepAdd_{t1-t2}, ConEco_{t1-t2})}{|DepAdd_{t1-t2}|}$
% \end{enumerate}

% Where $DepAdd_{t1-t2}$ is the Dependency add matrix and $ConEco_{t1-t2}$ is the Contributor matrix.

% %and $pkg$ $\in$ DCC~if $pkg.createDate$ $<$ $t1$.
% %We collect all $depends.types$ and $contributes.contributors$ that lie between $t1$ and $t2$ to construct our congruences.

% \begin{enumerate}[{\bf DC5:}]
%   \item DC$_{t1-t2}$ = $\frac{Match(DepAdd_{t1-t2}, ConDep_{t1-t2})}{|DepAdd_{t1-t2}|}$
% \end{enumerate}

% Where $DepAdd_{t1-t2}$ is the Dependency add matrix and $ConDep_{t1-t2}$ is the Dependent Maintainer matrix.

% \begin{enumerate}[{\bf DC6:}]
%   \item DC$_{t1-t2}$ = $\frac{Match(DepAdd_{t1-t2}, ConMaintain_{t1-t2})}{|DepAdd_{t1-t2}|}$
% \end{enumerate}

% Where $DepAdd_{t1-t2}$ is the Dependency add matrix and $ConMaintain_{t1-t2}$ is the Maintainer matrix.

% \begin{enumerate}[{\bf DC7:}]
%     \item DC$_{t1-t2}$ = $\frac{Match(DepRemove_{t1-t2}, ConEco_{t1-t2})}{|DepRemove_{t1-t2}|}$
% \end{enumerate}

% Where $DepRemove_{t1-t2}$ is the Dependency remove matrix and $ConEco_{t1-t2}$ is the Contributor matrix.


% \begin{enumerate}[{\bf DC8:}]
%   \item DC$_{t1-t2}$ = $\frac{Match(DepRemove_{t1-t2}, ConDep_{t1-t2})}{|DepRemove_{t1-t2}|}$
% \end{enumerate}

% Where $DepRemove_{t1-t2}$ is the Dependency remove matrix and $ConDep_{t1-t2}$ is the Dependent Maintainer matrix.

% \begin{enumerate}[{\bf DC9:}]
%   \item DC$_{t1-t2}$ = $\frac{Match(DepRemove_{t1-t2}, ConMaintain_{t1-t2})}{|DepRemove_{t1-t2}|}$
% \end{enumerate}

% Where $DepRemove_{t1-t2}$ is the Dependency remove matrix and $ConMaintain_{t1-t2}$ is the Maintainer matrix.

% \begin{enumerate}[{\bf DC10:}]
%     \item DC$_{t1-t2}$ = $\frac{Match(DepUpgrade_{t1-t2}, ConEco_{t1-t2})}{|DepUpgrade_{t1-t2}|}$
% \end{enumerate}

% Where $DepUpgrade_{t1-t2}$ is the Dependency upgrade matrix and $ConEco_{t1-t2}$ is the Contributor matrix.


% \begin{enumerate}[{\bf DC11:}]
%   \item DC$_{t1-t2}$ = $\frac{Match(DepUpgrade_{t1-t2}, ConDep_{t1-t2})}{|DepUpgrade_{t1-t2}|}$
% \end{enumerate}

% Where $DepUpgrade_{t1-t2}$ is the Dependency upgrade matrix and $ConDep_{t1-t2}$ is the Dependent Maintainer matrix.

% \begin{enumerate}[{\bf DC12:}]
%   \item DC$_{t1-t2}$ = $\frac{Match(DepUpgrade_{t1-t2}, ConMaintain_{t1-t2})}{|DepUpgrade_{t1-t2}|}$
% \end{enumerate}

% Where $DepUpgrade_{t1-t2}$ is the Dependency upgrade matrix and $ConMaintain_{t1-t2}$ is the Maintainer matrix.

% \begin{enumerate}[{\bf DC13:}]
%     \item DC$_{t1-t2}$ = $\frac{Match(DepDowngrade_{t1-t2}, ConEco_{t1-t2})}{|DepDowngrade_{t1-t2}|}$
% \end{enumerate}

% Where $DepDowngrade_{t1-t2}$ is the Dependency downgrade matrix and $ConEco_{t1-t2}$ is the Contributor matrix.


% \begin{enumerate}[{\bf DC14:}]
%   \item DC$_{t1-t2}$ = $\frac{Match(DepDowngrade_{t1-t2}, ConDep_{t1-t2})}{DepDowngrade_{t1-t2}|}$
% \end{enumerate}

% Where $DepDowngrade_{t1-t2}$ is the Dependency downgrade matrix and $ConDep_{t1-t2}$ is the Dependent Maintainer matrix.

% \begin{enumerate}[{\bf DC15:}]
%   \item DC$_{t1-t2}$ = $\frac{Match(DepDowngrade_{t1-t2}, ConMaintain_{t1-t2})}{|DepDowngrade_{t1-t2}|}$
% \end{enumerate}

% Where $DepDowngrade_{t1-t2}$ is the Dependency downgrade matrix and $ConMaintain_{t1-t2}$ is the Maintainer matrix.

%Where $E_D$ is the Ecosystem dependency matrix and $E_C_C$ is the Contributor contribution matrix.

% \christoph{Do we really need to mention packages when defining a time window? I would say that the time window is independent of whether packages, dependencies, developers, or anything else existed.}
% For the edge relationships, we capture the latest state that is between the time period (i.e., t1 $>$ E.time $>$ t2). \christoph{Mention this earlier. Also, how does this apply to the contribution relationships?}
% All other nodes and edges that do not appear during this time period are ignored. \christoph{... are not part of Gt1-t2? `ignored' sounds arbitrary.}

\begin{definition}[$E_{c}$ roles]
$E_{c}$ has two attributes <role, time> where the role, and time is when the contribution was made. 
The role refers to the access levels of the developer when making the contribution. There is only two types: a \texttt{maintainer}, who has the ability to merge any submitted contributions.
On the other hand, a \texttt{non-maintainer} can only submit contributions to a package, but does not have the ability to merge the package. 
Note that since a non-maintainer can become a maintainer in a different time frame, we specifically calculate the role at this point in time.
% We hypothesize that contributions that align to their dependencies is related to the role of the contributor.
\raula{probably need to clean this up later}
\christoph{I think it would be good to make it explicit what we do in cases where somebody was a maintainer and a non-maintainer in the same time frame}
\end{definition}
% \christoph{We need to define the terms maintainer and contributor here, and make it explicit that this list is exhaustive (it is, right?). Also, make it explicit what happens in the very likely event of multiple contributions from the same developer -- multiple edges, or multiple values for `time'?}

\begin{definition}[$E_{d}$ states]
$E_{d}$ has attributes <state, time> which is the current state of the dependency relationship.
To understand the current state of the a dependency at any point in time. They are (i) add, is that a dependency has just been added, (ii) remove is when the dependency has been removed from a package (iii) keep is when the package is still using an existing dependency (iv) upgrade is when a dependency version has a been changed to a more recent version and (v) downgrade is when a dependency version has been changed to a older version of a library.
% We hypothesize that there is a relationship between the change of dependency and a contribution that a library receives.
\raula{probably need to clean this up later}
\christoph{same comment: we should make it explicit what happens if multiple of these things happen in the same time frame}
\end{definition}

\begin{figure}
    \centering
    \scalebox{0.8}{
    \begin{tikzpicture}[
        roundnode/.style={circle, fill=black, minimum size=5mm},
        squarenode/.style={fill=black, text=red, minimum size=5mm},
    ]
    \begin{scope}
        
        \node[roundnode, label=right:$Pkg\_i$ as client] (s2_proji) at (4, 3) {};
        \node[roundnode, label=below:$Pkg\_j$ as library] (s2_projj) at (4,0) {};

        \node[squarenode, label=below:$Dev\_x$] (s3_devx) at (1.5, 1.5) {};
        
        
    \end{scope}

    \begin{scope} [every edge/.style={draw=black, very thick},
    every node/.style={fill=white}]
        \path [->] (s2_proji) edge[bend left=70] node {E$_{d}$} (s2_projj);
        
    \end{scope}
    \begin{scope} [every edge/.style={draw=gray, ultra thick, double distance=2pt},
    every node/.style={fill=white}]
        \path [->] (1.9, 1.5) edge[bend left=40] node {E$_{c}$} (s2_proji);
        \path [->] (1.9, 1.5) edge[bend right=40] node {E$_{c}$} (s2_projj);
    \end{scope}
    \end{tikzpicture}
    }
    \caption{Example of client and library contribution
    }
    \label{fig:clientlib}
\end{figure}

\subsection{Characterizing Contributor Roles and Dependencies}

As depicted in Figure \ref{fig:clientlib}, we use role attributes to now make an exhaustive list of all possible contribution combinations in terms of a client/library dependency relationship.
Based on this definition, we now list these exhaustive cases of developers that contribute to dependencies within the ecosystem  below:

% \paragraph{\textbf{Maintainer contributes to own dependency.}}
\begin{itemize}
    \item \textbf{\maintain} - Maintainer contributes to own client/library packages
This is the case where a maintainer will contribute to a library that they are also maintaining.
where $E.role = maintainer$ for  $N_{dev} \Rightarrow N_{pkg.j.}$ and $E.role = maintainer$ for  $N_{dev} \Rightarrow N_{pkg.i.}$
% \end{itemize}
% \paragraph{\textbf{Non-maintainer contributes to maintained dependency}}
% There are two types:
% \begin{itemize}
    \item {\textbf{\client} - \client contributes to a Library }
This is the case where a \client makes a contribution to a library that they depend on.
We also add the condition that the \client is not a maintainer of the library. This is 
where $E.role = contributor$ for  $N_{dev} \Rightarrow N_{pkg.j.}$ and $E.role = maintainer$ for  $N_{dev} \Rightarrow N_{pkg.i.}$
\item { \textbf{\library} - \library contributes to a client}
This is a case where the \library makes a contribution to a client package.
where $E.role = maintainer$ for  $N_{dev} \Rightarrow N_{pkg.j.}$ and $E.role = contributor$ for  $N_{dev} \Rightarrow N_{pkg.i.}$
\end{itemize}

% \paragraph{\textbf{Non-maintainers contribute to non-own dependency}}
\begin{itemize}
    \item 
 \textbf{\nonmaintain} - Ecosystem developer contribute to both library and client 
This is where a package receives contributions from developers not maintainers of the library or client package.
where $E.role = contributors $ for  $N_{dev} \Rightarrow N_{pkg.j.}$ and $E.role = contributor$ for  $N_{dev} \Rightarrow N_{pkg.i.}$
\end{itemize}


In terms of the contributions, we then split the groups based on whether they are contributed to their dependencies.

\begin{itemize}
    \item \textbf{\maintaincontribution (maintain)} - Taken from RQ1, ...\raula{complete}
    \item {\textbf{\clientcontribution (client)} } Taken from RQ1,
    \item \textbf{\nonmaintaincontribution (non-maintain)} - As a baseline, we then collect all other contributions from the contributor.
\end{itemize}

\christoph{I'm confused how these definitions relate to the ones in Section 2. Are they `just' giving names to phenomena that you could define given the information from Section 2, or does this add something that's not covered in Section 2?}


\subsection{Temporal Attributes}
Using these attributes, we can now analyze the state of contributions and dependencies at any given period in time.
Hence, we define a timed $G$, $G_{t1-t2}$ where t1 and t2 are two points in time. Formally:
\begin{equation}
    G_{t1-t2} = (N_{t1-t2}, E_{t1-t2})
\end{equation}

where t1 captures any nodes and edges within a given time frame. \christoph{why does t1 capture these? shouldn't it be t1-t2?}
This captures any package created before a time-frame.
Hence for any time period (t1 to t2), the timed graph will capture any packages and developers that were created before the time period (i.e., 
$N_{pkg}.time < t1$). 
In terms of E$_{t1-t2}$, we only consider contributions $t1 < E_{c}.time < t2$ and dependency states $t1 < E_{d}.time < t2$ that were recorded during this time period.
For example, .... \raula{we need to add an example.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
\begin{subfigure}{\linewidth}
    \centering
    \scalebox{0.7}{
    \begin{tikzpicture}[
        roundnode/.style={circle, fill=black, minimum size=5mm},
        squarenode/.style={fill=black, text=red, minimum size=5mm},
    ]
    \begin{scope}
        
        \node[roundnode, label=above:$N_{pkg.i}$] (s2_proji) at (3, 2.5) {};
        \node[roundnode, label=below:$N_{pkg.j}$] (s2_projj) at (4,0) {};
        \node[roundnode, label=below:$N_{pkg.k}$] (s2_projk) at (2,0) {};
      
        \node[squarenode, label=below:$N_{dev.x}$] (s3_devx) at (6, 1.25) {};
        
        
    \end{scope}

    \begin{scope} [every edge/.style={draw=gray, very thick}]
        \path [->] (s2_proji) edge (s2_projj);
        \path [->] (s2_proji) edge (s2_projk);
        \path [->] (s2_projj) edge (s2_projk);
     
    \end{scope}
    \begin{scope} [every edge/.style={draw=gray, thick, double distance=2pt}]
        %\path [->] (6, 2.8) edge (s2_proji);
        %\path [->] (6, 2.8) edge[bend left=15] (s2_projj);
        \path [->] (5.7, 1.25) edge (s2_proji);
        \path [->] (5.65 , 1.25) edge (s2_projj);
    
    \end{scope}
    \end{tikzpicture}
    }
    \caption{Before the first quarter of 2016}
    \label{fig:graph_before}
\end{subfigure}
\begin{subfigure}{\linewidth}
    \centering
    \scalebox{0.7}{
    \begin{tikzpicture}[
        roundnode/.style={circle, fill=black, minimum size=5mm},
        squarenode/.style={fill=black, text=red, minimum size=5mm},
    ]
    \begin{scope}
        
        \node[roundnode, label=right:$N_{pkg.i}$] (s2_proji) at (4, 1.5) {};
        \node[roundnode, label=below:$N_{pkg.j}$] (s2_projj) at (5,0) {};
        \node[roundnode, label=below:$N_{pkg.k}$] (s2_projk) at (3,0) {};
        
        \node[squarenode, label=below:$N_{dev.x}$] (s3_devx) at (2, 3.5) {};
        
        \node[squarenode, label=below:$N_{dev.y}$] (s3_devy) at (6, 3.5) {};
        
    \end{scope}

    \begin{scope} [every edge/.style={draw=gray, very thick}]
        \path [->] (s2_proji) edge (s2_projj);
        \path [->] (s2_proji) edge (s2_projk);
        \path [->] (s2_projj) edge (s2_projk);
        
    \end{scope}
    \begin{scope} [every edge/.style={draw=gray, thick, double distance=2pt}]
        \path [->] (6, 2.8) edge (s2_proji);
        \path [->] (6, 2.8) edge[bend left=15] (s2_projj);
        \path [->] (2, 2.8) edge (s2_proji);
        \path [->] (2, 2.8) edge[bend right=15] (s2_projk);
    \end{scope}
    \end{tikzpicture}
    }
    \caption{During  the first quarter of 2016 (i.e.,  January 1 to March 31 2016)}
    \label{fig:graph_in_period}
\end{subfigure}
\caption{Example graph representation of the relationships between contributions and dependencies.}
 \label{fig:graph}
\end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \christoph{I would show the matrices for these four scenarios. As far as I can see, two small matrices (one for dependencies, one for contributions) should be sufficient to show this, right? Also, can we make it explicit that this covers all possible contributions?}

% We can represent the edges as a matrix as below

%  \begin{gather}
%   E_{depends}
%  =
%   \begin{bmatrix}
%   N_{pkg.i} &
%   N_{pkg.j} \\
%   N_{pkg.j} &
%   N_{pkg.k} 
%   \end{bmatrix}
% \end{gather}


%  \begin{gather}
%   E_{contribute}
%  =
%   \begin{bmatrix}
%   N_{pkg.i} &
%   N_{pkg.j} \\
%   N_{pkg.j} &
%   N_{pkg.k} 
%   \end{bmatrix}
% \end{gather}

% at where pkg.time and E.time \raula{has to fix up later}.
% For each $pkg$, we have the following unique attributes:
% \begin{itemize}
%     \item pkg.name
%     \item pkg.createdDate
% \end{itemize}

% We now highlight the following relationships between other packages in the ecosystem:
% \begin{itemize}
%     %\item depends (type)  - types include add, update, downgrade, and remove.
%     \item depends (dependency, dependencyChange) - dependency includes $pkg$ dependencies' name, and dependencyChange includes change histories of the $pkg$ dependencies. The change types consist of exist, add, update, downgrade, and remove.
    
%     \christoph{It'll be difficult to explain that `remove' is a type of dependency. Can we separate the static and dynamic aspects of this, i.e., have a `dependencyChange' and a `dependency'? Also, do we need the time frame discussion here already?}
%     \item contributes (type) - type includes maintainer and contributor.
%     We define a maintainer as a user who can merge pull request commits, and submitted at least one pull request or opened at least one issue in the $pkg$. \christoph{do you mean pull request? This part is unclear -- X or X and X?}. A contributor is a user who submitted at least one pull request or opened at least one issue in the $pkg$ but he or she is not the owner and in the maintainer list of the $pkg$. \christoph{This does not appear to be exhaustive: what about a person who is in the maintainer list but has never done anything?}
% \end{itemize}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[t]
% \centering
% \begin{tikzpicture}
% \begin{scope}[every node/.style={thick,draw}]
%     \node (pkgj) at (2,0) {$pkg_j$};
%     \node (pkgk) at (-3,2) {$pkg_k$};
%     \node (pkgi) at (0,4) {$pkg_i$};
%     \node (pkgl) at (-3,0) {$pkg_l$};
% \end{scope}
% \begin{scope}[>={Stealth[black]},
%               every node/.style={fill=white},
%               every edge/.style={draw=blue,very thick}]

% \path [->] (pkgi) edge[bend right=-90] node {dep (has, add, remove, upgrade, downgrade)} (pkgj);
% \end{scope}
% \begin{scope} [>={Stealth[black]},
% every node/.style={fill=white},
% every edge/.style={draw=red, very thick}]
% \path [->] (pkgi) edge[bend right=-10] node {contribute(co-maintain)} (pkgj);
% \path [->] (pkgi) edge[bend left=-80] node {contribute(depend)} (pkgj);
% \path [->] (pkgk) edge[bend right=30] node {contribute(transitive)} (pkgj);
% \end{scope}
% \begin{scope} [>={Stealth[black]}, dashed,
% every node/.style={fill=white},
% every edge/.style={draw=red, very thick}]
% \path [->] (pkgk) edge[bend right=-30] node {} (pkgi);
% \end{scope}
% \begin{scope} [>={Stealth[black]}, dashed,
% every node/.style={fill=white},
% every edge/.style={draw=grey, very thick}]
% \path [->] (pkgl) edge[bend right=30] node {contribute(ecosystem)} (pkgj);
% \end{scope}
% \end{tikzpicture}
% \caption{The different dependencies and contributions between packages in the ecosystem}
% \label{fig:relationships}
% \end{figure}



% \begin{figure}[]
%     \centering
% \begin{subfigure}{\linewidth}
% \centering
% \begin{tikzpicture}
% \begin{scope}[every node/.style={thick,draw}]
%     \node (pkgj) at (2,0) {$pkg_j$};
%     \node (pkgi) at (0,4) {$pkg_i$};
%     \node (ux) at (-2,2) {$u_x$};
% \end{scope}
% \begin{scope}[>={Stealth[black]},
%               every node/.style={fill=white},
%               every edge/.style={draw=blue,very thick}]

% \path [->] (pkgi) edge[bend right=-90] node {depends(add, remove, upgrade, downgrade)} (pkgj);
% \end{scope}
% \begin{scope} [>={Stealth[black]}, dashed,
% every node/.style={fill=white},
% every edge/.style={draw=blue, very thick}]
% \path [->] (pkgi) edge[bend right=-15] node {depends(has)} (pkgj);
% \end{scope}
% \begin{scope} [>={Stealth[black]},
% every node/.style={fill=white},
% every edge/.style={draw=red, very thick}]
% \path [->] (ux) edge[bend right=-50] node {\textbf{maintainer}} (pkgi);
% \path [->] (ux) edge[bend left=-50] node {\textbf{contributor}} (pkgj);
% \end{scope}
% \end{tikzpicture}
% \caption{An illustrative example.}
% \label{fig:example_contribute-d}
% \end{subfigure}
% \begin{subfigure}{\linewidth}
% \centering
% \begin{matrix}
%  & $pkg_i$ & $pkg_j$\\
% $pkg_i$ & 0 & 1 \\
% $pkg_j$ & 0 & 0
% \end{matrix}
% \caption{A contribute-d matrix based on the illustrative example.}
% \end{subfigure}
% \label{fig:relationships_contribute-d}
% \caption{The different dependencies and dependent package contributions (contribute-d) between packages in the ecosystem.}
% \end{figure}



% \begin{figure}[]
%     \centering
% \begin{subfigure}{\linewidth}
% \centering
% \begin{tikzpicture}
% \begin{scope}[every node/.style={thick,draw}]
%     \node (pkgj) at (2,0) {$pkg_j$};
%     \node (pkgi) at (0,4) {$pkg_i$};
%     \node (pkgk) at (-3,0) {$pkg_k$};
%     \node (ux) at (-2,2) {$u_x$};
% \end{scope}
% \begin{scope}[>={Stealth[black]},
%               every node/.style={fill=white},
%               every edge/.style={draw=blue,very thick}]

% \path [->] (pkgi) edge[bend right=-90] node {depends(add, remove, upgrade, downgrade)} (pkgj);
% \end{scope}
% \begin{scope} [>={Stealth[black]}, dashed,
% every node/.style={fill=white},
% every edge/.style={draw=blue, very thick}]
% \path [->] (pkgi) edge[bend right=-15] node {depends(has)} (pkgj);
% \end{scope}
% \begin{scope} [>={Stealth[black]},
% every node/.style={fill=white},
% every edge/.style={draw=red, very thick}]
% \path [->] (ux) edge[bend right=-50] node {\textbf{contributor}} (pkgi);
% \path [->] (ux) edge[bend left=-50] node {\textbf{contributor}} (pkgj);

% \end{scope}
% \begin{scope} [>={Stealth[black]}, dashed,
% every node/.style={fill=white},
% every edge/.style={draw=red, very thick}]
% \path [->] (ux) edge[bend left=-50] node {} (pkgk);
% \end{scope}
% \end{tikzpicture}
% \caption{An illustrative example.}
% \label{fig:example_contribute-e}
% \end{subfigure}
% \begin{subfigure}{\linewidth}
% \centering
% \begin{matrix}
%  & $pkg_i$ & $pkg_j$\\
% $pkg_i$ & 0 & 1 \\
% $pkg_j$ & 0 & 0
% \end{matrix}
% \caption{A contribute-e matrix based on the illustrative example.}
% \end{subfigure}
% \caption{The different dependencies and ecosystem contributions (contribute-e) between packages in the ecosystem.}
% \label{fig:relationships_contribute-e}
% \end{figure}


% \subsection{Four types of Contributions}

% We describe the dependencies and contributions as package-by-package matrices.
% % \paragraph{\texttt{depends} Matrices:}
% We now define the matrices from t1 time to t2, where $pkg$ $\in$ package-by-package matrices~if $pkg.createDate$ $<$ $t1$.
% % We then collect all $depends.types$ and $contributes.contributors$ that lie between $t1$ and $t2$ to construct Dependency between packages and contribution between packages matrices.
% \begin{definition}[Depends matrices]
% We first describe the dependency relationship.
% \begin{equation}
%     depends(i,j,type)_{t1-t2}
% \end{equation}
% where $type$ is that is the different types of dependencies. Here, $depends_i_j$ is an element in $depends_{t1-t2}$, $depends_i_j$ = 1 means that $pkg_i$ depends on $pkg_j$ from t1 to t2 with the $type$ (i.e., exist, add, remove, upgrade, and downgrade).
% \end{definition}

% \begin{gather}
%  \begin{bmatrix} \Phi_{11} & \Phi_{12} \\ \Phi_{21} & \Phi_{22} \end{bmatrix}
%  =
%  \frac{1}{\det(X)}
%   \begin{bmatrix}
%   X_{22} Y_{11} - X_{12} Y_{21} &
%   X_{22} Y_{12} - X_{12} Y_{22} \\
%   X_{11} Y_{21} - X_{21} Y_{11} &
%   X_{11} Y_{22} - X_{21} Y_{12} 
%   \end{bmatrix}
% \end{gather}

% \christoph{Could we simplify to depends(i, j, type)? I'm not sure why i and j are currently subscripts while the x is in brackets?}

% Figure \ref{fig:relationships} illustrates the relationship among packages that we use to construct the package-by-package matrices and compute congruences.
% According to the Dependency-contribution congruence, when $pkg_i$ depends on, adds, removes, upgrades, or downgrades $pkg_j$ (depicting in the Dependency between packages matrices). 
% % % \begin{enumerate}[{\bf Dep:}]
% % % \item  
% % % \end{enumerate}
% % %\item Dependency update matrix ($E_D_U$): if $edu_i_j$ is an element in $E_D_U$, $edu_i_j$  = 1 means that $pkg_i$ updates (i.e., adds, removes, upgrades, or downgrades) $pkg_j$.
% % \begin{definition}[$DepAdd_{t1-t2}$]
% % A Dependency add matrix is $add_i_j$ is an element in $DepAdd_{t1-t2}$, $add_i_j$  = 1 means that $pkg_i$ adds $pkg_j$ during the period between t1 and t2.
% % \end{definition}
% % \begin{definition}[$DepRemove_{t1-t2}$]
% % A Dependency remove matrix is $remove_i_j$ is an element in $DepRemove_{t1-t2}$, $remove_i_j$  = 1 means that $pkg_i$ removes $pkg_j$ during the period between t1 and t2.
% % \end{definition}
% % \begin{definition}[$DepUpgrade_{t1-t2}$]
% % A Dependency upgrade matrix is $upgrade_i_j$ is an element in $DepUpgrade_{t1-t2}$, $upgrade_i_j$  = 1 means that $pkg_i$ upgrades $pkg_j$ during the period between t1 and t2.
% % \end{definition}

% % \begin{definition}[$DepDowngrade_{t1-t2}$]
% % A Dependency downgrade matrix is $downgrade_i_j$ is an element in $DepDowngrade_{t1-t2}$, $downgrade_i_j$  = 1 means that $pkg_i$ downgrades $pkg_j$ during the period between t1 and t2.
% % \end{definition}
% Similarly, we characterize the different contributions into three types.
% The first contribution are contributions that come from the ecosystem and not from $pkg_i$.

% \begin{definition}[contribution matrices]
% \begin{equation}
%     contribute(y)_{t1-t2}
% \end{equation}
% where $y$ is the different types of contribution. Here, $contribute_i_j$ is  an element in \sloppy{($contribute_{t1-t2}$)} , $contributes_i_j$  = 1 
% means that a contributor to $pkg_i$ and $pkg_j$, made at least one contribution to $pkg_j$ during the period between t1 and t2 with the type $y$ (i.e., contribute-e, contribute-m and contribute-d.
% \end{definition}

% % \begin{definition}[$contribute-d_{t1-t2}$]
% % A Dependent Maintainer matrix is $cdep_i_j$ is an element in ($contribute-d_{t1-t2}$), $cdep_i_j$ =1 means that a maintainer of only $pkg_i$, made at least one contribution to $pkg_j$ during the period between t1 and t2.
% % \end{definition}
% % \begin{definition}[$contibute-m_{t1-t2}$]
% % A Maintainer matrix is $cmaintain_i_j$ is an element in ($contribute-m_{t1-t2}$), $cmaintain_i_j$  = 1 means that a co-maintainer of $pkg_i$ and $pkg_j$, made at least one contribution to $pkg_j$ during the period between t1 and t2.
% % \end{definition}
% %  $pkg_j$ should get contributions from the dependent $pkg_i$ (depicting in Dependent maintainer matrix), from co-maintainers of $pkg_i$ and $pkg_j$ (depicting in maintainer matrix), add/or from ecosystem (depicting in contributor matrix), e.g., $pkg_k$.


\subsection{Congruence Calculation}
We now represent the graphs as adjacency matrix representations. 
First we would like to extract and represent the timed graph $G_{t1-t2} \in \{ N_{pkg.i}, N_{pkg.j}, ...N_{pkg.k}\}$  \christoph{Doesn't the `in' relationship need to go the other way?}

% \christoph{Do we need to mention the time window here and make it a parameter of the matrices?}
\begin{definition}[$C_E$ adjacency matrix]
We first define contributions between two package as a matrix where $C_E$ is a |$N_{pkg}$| x |$N_{pkg}$| 2D square matrix with its element represents $\{pkg_{i,j} |i,j \in  \{N_{dev} \Rightarrow N_{pkg.i} \wedge N_{dev} \Rightarrow N_{pkg.j} $where $  pkg_{i,j} \in G_{t1-t2} \}$. 
% If there is no contributions between the packages \christoph{I think we need to be more precise here. If there is no developer who has contributed to both?}, then matrix representation is zero. Note that dependency edges are ignored.
As a running example, Figure \ref{fig:graph} is represented as a matrix below: 
% \christoph{Since the relationship is indirect, I think we should explain the values, in particular which developer accounts for which value. Also, should we make it explicit that we ignore weights, e.g., how many developers contributed to both and/or how many contributions they made?}
\[
\begin{blockarray}{cccccc}
 &N_{pkg.i} & N_{pkg.j} & N_{pkg.k} \\
\begin{block}{c[ccccc]}
N_{pkg.i} & 0 & 1& 1 \bigstrut[t] \\
N_{pkg.j} & 1 &0 & 0 \\
N_{pkg.k} & 1 &0 & 0 \bigstrut[b]\\
\end{block}
\end{blockarray}\vspace*{-1.25\baselineskip}
\]
\end{definition}

where there is a developer ($N_{dev.y}$) who had contributed to two different packages (i.e., $N_{pkg.i}$, $N_{pkg.j}$ and $N_{pkg.i}$, $N_{pkg.k}$).
The values of the matrix are either zero or one, to show whether there was a contribution between two packages at a time period (i.e., t1 and t2). 


\begin{definition}[$C_D$ adjacency matrix]
To align the contribution between two packages with a dependency, we define $C_D$ as a |$N_{pkg}$| x |$N_{pkg}$| 2D square matrix with its element represents $\{pkg_i,k |i,k \in  N_{pkg.i} \rightarrow N_{pkg.j} $where $  pkg_i,j \in G_{t1-t2} \}$. 
For $C_D$ $\in G_{t1-t2}$, as shown in Figure \ref{fig:graph} is represented as:
\[
\begin{blockarray}{cccccc}
 & N_{pkg.i} & N_{pkg.j} & N_{pkg.k} \\
\begin{block}{c[ccccc]}
N_{pkg.i} & 0 & 1& 1 \bigstrut[t] \\
N_{pkg.j} & 0 &0 & 1  \\
N_{pkg.k} & 0 &0 & 0  \\
\end{block}
\end{blockarray}\vspace*{-1.25\baselineskip}
\]
\end{definition}
showing the dependencies of $N_{pkg.i} \rightarrow N_{pkg.j}$, $N_{pkg.j} \rightarrow N_{pkg.j}$, and $N_{pkg.j} \rightarrow N_{pkg.k}$
Note that the values of the matrix are either zero or one, to determine whether is a dependency or not at a time period (i.e., t1 and t2). \christoph{how does this relate back to the different states mentioned in Definition 2.3.2?}

\begin{definition}[EcosystemC] 
% \christoph{Why are these called STC? Just C would be sufficient, right?}
Taking these two adjecent matrix, we are now able to calculate the congruence between the dependency and the contribution for the graph of contribution and dependencies (i.e., $G_{t1-t2}$ for a given time period), which is based on socio-technical congruence as defined by Wagstrom \cite{wagstrom2010communication}.
% \christoph{Maybe mention that this is the same as previous work? i.e., similar to the next one.}
\begin{equation}
\begin{multlined}
   EcosystemC(G_{t1-t2}) = \\ 
    % \frac{(N_{pkg.i} \rightarrow N_{pkg.j})_{t1-t2}, N_{dev} \Rightarrow N_{pkg.j})}{|(N_{pkg.i} \rightarrow N_{pkg.j})_{t1-t2}|} \\
    = \frac{\Sigma (C_D \wedge C_E)}{\Sigma C_D}
\end{multlined}
\end{equation}

Given the example $C_D$ and $C_E$ adjacency matrices, we calculate the congruence as:

\[EcosystemC(G_{example})  = \frac{2}{3} = 0.6667 \]

In the example, the $C_D$ matrix shows 3 pairs of package dependencies, which are $N_{pkg.i} \rightarrow N_{pkg.j}$, $N_{pkg.j} \rightarrow N_{pkg.j}$, and $N_{pkg.j} \rightarrow N_{pkg.k}$.
The $C_E$ matrix shows that there are 2 pairs of contributions between two packages congruent with those package dependencies, which are $N_{pkg.i} \Rightarrow  N_{pkg.j}$ and $N_{pkg.i} \Rightarrow  N_{pkg.k}$.
Thus, the resulting congruence for this example is 0.667.
 
\christoph{Should we add the individual package congruence definition here as well? Might be good to have all definitions in one place}

% \raula{we have to make this a generalized definition, so that we can insert any of the matrices into it.}
% Subsequently, we use the same algorithm to calculate for DepAdd, DepRemove, DepUpgrade and DepDowngrade for the different contributions (i.e., contribute-e, contribute-d and contribute-m).
\end{definition}


\begin{definition}[PkgC]
Taking into consideration the studies by Wagstrom \cite{doi:10.5465/ambpp.2010.54500789}, the individual package congruence can be defined as follow. 
\begin{equation}
\begin{multlined}
   PgkC(G_{t1-t2}, i) = \\ \frac{ \Sigma (C_{D}[i,] \wedge C_{E}[i,])  + \Sigma (C_{D}[,i] \wedge C_{E}[,i])}{\Sigma (C_{D}[i,] + \Sigma (C_{D}[,i]}
\end{multlined}
\end{equation}
where $i$ is any N$_{pkg}$ within a given time period (i.e., t1 and t2).
The numerator of the equation calculates the number of contribution activities correspond to dependencies of N$_{pkg}$, considering only the rows and columns of the matrix corresponding to N$_{pkg}$.
\end{definition}

\raula{lets make a example of the individual package congruence}






==> sections/OLDsetup.tex <==





